Non-Count Symmetries in Boolean & Multi-Valued Prob. Graphical Models

Lifted inference algorithms commonly exploit symmetries in a probabilistic graphical model (PGM) for efficient inference. However, existing algorithms for Boolean-valued domains can identify only those pairs of states as symmetric, in which the number of ones and zeros match exactly (count symmetries). Moreover, algorithms for lifted inference in multi-valued domains also compute a multi-valued extension of count symmetries only. These algorithms miss many symmetries in a domain. In this paper, we present first algorithms to compute non-count symmetries in both Boolean-valued and multi-valued domains. Our methods can also find symmetries between multi-valued variables that have different domain cardinalities. The key insight in the algorithms is that they change the unit of symmetry computation from a variable to a variable-value (VV) pair. Our experiments find that exploiting these symmetries in MCMC can obtain substantial computational gains over existing algorithms.

==> taxonomy.tex <==
\section{A Taxonomy of State Symmetries}
In this section, we describe a taxonomy of symmetries over a family of graphical models. In our taxonomy, we gradually move from coarser notions of symmetry to more finer notions. The discussion in this section will also lay the foundation for the symmetry types that we describe later in this paper. We start with some definitions.

In the discussion below, we will assume that our models are defined over a finite set of discrete valued variables $\mathcal{X}$ where each $X_i \in \mathcal{X}$ has a domain $D_i$. Consider a set of indexes $\{1,2,\cdots,m\}$. Let $\mathcal{I}=\{I_l\}_{l=1}^{k}$ denote a partition of this index set into $k$ disjoint subsets. Each $I_l$ denotes a subset of indexes and $I_{l}$ and $I_{l'}$ are disjoint whenever $l \neq l'$.
\begin{defn}
Given a partition $\mathcal{I}$ of an $m$-sized index set, let $\mathcal{F_I}$ denote a family of graphical models $\{\mathcal{G}({\bf w})\}$ parameterized by the weight vector ${\bf w}$ where each $\mathcal{G}({\bf w})$ takes the form of the set of pairs $\{f_j,w_j\}_{j=1}^{m}$, ${\bf w}$ denoting the vector of weights $(w_1,w_2,\cdots,w_m)$. The weight vector ${\bf w}$ respects the \markred{partition $I$} %RN: Is it suppose to be \mathcal{I} here?
in the sense such that if $j,j' \in I_l$ for some $l$, then $w_j=w_{j'}$.
\end{defn}
As an example, a set of Markov logic networks (MLN)~\cite{domingos&lowd09} where MLNs in the set have a fixed set of formulas but differ on the formula weights can be seen as generating a family of graphical models where all the groundings of a first-order logic formula have the same weight.

We will talk about symmetries over a family of graphical models as defined above. In order to keep our formulation general enough, instead of defining them via permutations that preserve the graph structure, we will first define them in terms of probability preserving permutations over the underlying state space. We will then describe how these broader notions of symmetry relate to those discovered using the graph structure. \bug{Need to talk about how we related to Bui's 2013 paper on automorphism groups}
\begin{defn}
Let $\mathcal{F_I}$ represent a family of graphical models. Let $\psi$ denote a permutation over the state space $\mathcal{S}$. We say that $\psi$ is a {\em state symmetry} of the family $\mathcal{F_I}$ if $\forall \mathcal{G}$ belonging to the family, $P_{\mathcal{G}}(s)=P_{\mathcal{G}}(\psi(s))$.
\end{defn}
\begin{thm}
Set of all state symmetries of a family $\mathcal{F_I}$ forms a permutation group. We will denote this permutation group by $\Psi^{*}$.
\end{thm}
Note that $\Psi^{*}$ partitions the set of states $\mathcal{S}$ into a set of orbits where the orbit of a state $s \mathcal{S}$ is given by $\Gamma_{\psi^{*}}(s)$. In some sense, $\Psi^{*}$ gives us the finest possible notion of symmetry for a given family of graphical models. In general, we believe that computing $\Psi^{*}$ is intractable therefore, we have to work with coarser partitions of the state space. 
\begin{defn}
Let $\Psi_1$ and $\Psi_2$ denote two permutation groups over state symmetries. We say that $\Phi$ is a coarser symmetry group over ${\mathcal S}$ than $\Phi_2$, if $\forall s \in \mathcal{S}$, we have $\Gamma_{\Psi_1}(s) \subseteq \Gamma_{\Psi_2}(s)$. We also say that $\Psi_2$ is a finer symmetry group than $\Psi_2$.
\end{defn}
Before we go any further, we will find the following notation useful. Given a set of variables $X \subseteq \mathcal{X}$ sharing the same domain $D_{X}$ and a $v \in D_{X}$, $count_{X}(s,v)$ computes the number of variables in set ${\bf X}$ taking the value $v$ in the state $s$. We are now ready to describe a taxonomy of state symmetry which goes from coarser to finer.
\begin{itemize}
\item {\bf Count Symmetries:} A state symmetry $\psi$ is a count symmetry if for each subset $X \subseteq \mathcal{X}$ having the same domain $D_{\bf X}$, $count_{X}(s,v)=count_{X}(s',v)$, $\forall v \in D_{X}$. Note that for Boolean domains count symmetries translate to having the same number of 1's (or $0$'s) in $s$ and $s'$. We say that a symmetry group $\Psi$ is a {\em count symmetry group} if every $\psi \in \Psi$ is a count symmetry. It is easy to see that symmetries computed by permuting variables (such as those described in Section~\ref{sec:background}) must be count symmetries. Most existing work on symmetries deals with count symmetries since they operate of variable permutations. 

\item  {\bf Count Symmetries after Single Renaming of Values (SRV-Count)}: This is a natural extension of count symmetries. Given a domain $D_i$, we say that $D'_i$ is a renaming of $D_i$
if there exists a bijection between $D_i$ and $D'_i$. We say that a symmetry group $\Psi$ is a {\ em SRV-count symmetry} group if there exists a renaming $D'_i$ of domain $D_i$ for every variable $X_i$, such that $\psi \in \Psi$ is a count symmetry after the domains have been renamed. Note that count symmetry group is a special case of SRV-count where the renaming transformation is identity.

For example, the two symmetric states of PGM $\G_1$ (defined above) are $(a=0, b=0)$, and $(a=1, b=1)$. These can be represented via count symmetries if we rename $b.0$ to $b.1$ and $b.1$ to $b.0$. In general, we believe that finding an optimal renaming (which results in most count symmetries) is intractable.

{\bf 3. Count Symmetries after taking Union of Renaming of Values (URV-Count):} This is a generalization of SRV-count symmetry group. We say that $\Psi$ is a URV-Count symmetry group if every $\psi \in \Psi$ is a count symmetry under some possible renaming of the domains. For example, consider $\G_3$ over Boolean variables $a$ and $b$ with a single formula $w:$ $a \oplus b$, where $\oplus$ represents the xor operator. It is easy to see that the state partition induced by $\Psi*$ is $\{(0,1), (1,0)\}$, and $\{(0,0), (1,1)\}$. Symmetry computation over any single renaming can not induce these orbits simultaneously via count symmetries --  the original domain can compute the first one, and renaming $b.0=b.1$ and $b.1=b.0$ can compute the second one. However, the union of symmetries under both these renamings captures all the desired symmetries. The VV symmetries described in Section~\ref{sec:vv} fall under this category.

{\bf 4. Equicardinal Symmetries: } This represents the complete class of symmetries in which a variable can only be mapped to other equicardinal variables. This raises the question: are there equicardinal symmetries which are not union of SRV count symmetries. Yes, there are! An example, is domain $\G_2$ (defined above). It is easy to see that its symmetric orbit contains states $(0, Dark), (1, Light)$, and $(1, Dark)$. Count symmetries over the renaming $X_2.Light = 0, X_2.Dark = 1$ can identify that states $(0, Dark)$ and $(1, Light)$ are symmetric. Unfortunately, no renaming can merge either of these states with $(1, Dark)$. This particular symmetry is a contextual symmetry \cite{anand&al16}, which is a symmetry notion orthogonal to VV symmetries.

{\bf 5. Non-equicardinal Symmetries: } This symmetry type caters to permutations between variables that need not even have the same cardinality of domains. This is discussed in detail in Section \ref{sec:nonequi}.
\end{itemize}

While our symmetry types are by no means meant to be exhaustive, to the best of our knowledge, it is the first attempt towards a taxonomy of symmetry classes in PGMs. Moreover, we are able to characterize the VV symmetries that we can compute in terms of this taxonomy.
%This is an important symmetry type in which a symmetry can be computed via a union of multiple count symmetries after different single renamings of values. Here, the union operator will merge all orbits involving any common state. For example, consider $\G_3$ over Boolean variables $a$ and $b$ with two formulas $w1:$ $a \oplus b$, and $w2:$ $\neg(a \oplus b)$, where $\oplus$ represents the xor operator. It is easy to see that its orbits are $\{(0,1), (1,0)\}$, and $\{(0,0), (1,1)\}$. No single renaming can represent both these orbits simultaneously via count symmetries --  the original domain can compute the first one, renaming $b.0=1$ and $b.1=0$ can compute the second one. However, the union of both can compute all the symmetries in the domain.




%We have already demonstrated that VV symmetries is a much more general representation of PGM symmetries than variable symmetries. We now explore the varieties of symmetries of a PGM in some more detail, and develop a taxonomy of symmetry types. In our taxonomy each successive symmetry type is more general than all preceding symmetry types. 

%It is helpful to visualize any symmetry via the state space partition induced by its orbits. A brute-force approach for computing {\em all} symmetries of a graphical model $G$ is to compute the joint probability of each state and combine all states with the same value into an orbit.\footnote{This joint probability must be computed algebraically using weights as variables (instead of specific numeric values) -- thus allowing the symmetry to be applicable to all PGMs with that structure, irrespective of exact weight values for each feature.} Let this be represented as a partition $\mathcal{P}^* = \{C^*_1, C^*_2, \ldots, C^*_{|\mathcal{P}^*|}\}$ over the whole state space $\mathcal{S}$, where each $C_i=\{s^i_1, s^i_2,\ldots, s^i_{|C_i|}\}$. Any other sound (but incomplete) symmetry of $\G$ will then induce a partition $\mathcal{P}=\{C^\mathcal{P}_1, C^\mathcal{P}_2, \ldots, C^\mathcal{P}_{|\mathcal{P}|}\}$ \markred{such $\mathcal{P}$ is a finer partition of $\mathcal{P^*}$}. In other words,  $\forall i\in\{1...|\mathcal{P}|\}$, there exists a unique $j\in \{1...|\mathcal{P^*}|\}$ s.t., $s\in C^\mathcal{P}_i \implies s\in C^*_j$.%RN: Wouldn't it be simpler to say that P is a finer partition of P^*?

%Since computing all symmetries of a PGM is intractable \bug, various methods (e.g. \cite{niepert12,anand&al16}) compute  sound but incomplete symmetries. What kinds of symmetries do they compute? To characterize this, we define the following symmetry types:

%{\bf 1. Count Symmetries: }  We call an automorphism group a count symmetry if, for each of its orbits, the number of 1s and 0s (in a Boolean-valued domain) are the same for all states in that orbit. To define the analogous concept for a multi-valued PGM, we will first cluster all variables into  subsets based on their domains. A symmetry is a count symmetry if, for each of its orbits, the number of occurrences of each discrete value \markred{in any such subset} %RN: Did this phrase come in by mistake? What did you mean by subset?
%is the same for all states in that orbit. 

%It is easy to see that variable automorphism groups can only compute count symmetries, since by permuting variables the count of each value always remains the same.

%{\bf 2. Count Symmetries after Single Renaming of Values (SRV): } This symmetry type is a natural extension in which symmetries are count symmetries after \markred{renaming values of each variable to some possibly new values}. %RN: Maybe plural would be better: "renaming values of each variable to some possibly new values"
%For example, the two symmetric states of PGM $\G_1$ (defined above) are $(a=0, b=0)$, and $(a=1, b=1)$. These can be represented via count symmetries if we rename $b.0$ to $1$ and $b.1$ to $0$. We believe that computing the optimal renaming that achieves the best symmetries will be intractable\bug. 

%{\bf 3. Union of SRV Count Symmetries: } This is an important symmetry type in which a symmetry can be computed via a union of multiple count symmetries after different single renamings of values. Here, the union operator will merge all orbits involving any common state. For example, consider $\G_3$ over Boolean variables $a$ and $b$ with two formulas $w1:$ $a \oplus b$, and $w2:$ $\neg(a \oplus b)$, where $\oplus$ represents the xor operator. It is easy to see that its orbits are $\{(0,1), (1,0)\}$, and $\{(0,0), (1,1)\}$. No single renaming can represent both these orbits simultaneously via count symmetries --  the original domain can compute the first one, renaming $b.0=1$ and $b.1=0$ can compute the second one. However, the union of both can compute all the symmetries in the domain.





